Local Variables and Quantum Relational Hoare Logic

We add local variables to quantum relational Hoare logic (Unruh, POPL 2019). We derive reasoning rules for supporting local variables (including an improved "adversary rule"). We extended the qrhl-tool for computer-aided verification of qRHL to support local variables and our new reasoning rules.

==> macros.tex <==
\makeatletter

\newcommand\pagelabel[1]{\phantomsection\label{#1}}

\newcommand\lemmalabel[1]{\label{#1}\def\@lemmalabel@current{#1}}
\newcommand\itlabel[1]{\csxdef{@itemlabel@lemma-#1}{\@lemmalabel@current}\label{#1}}
\newcommand\lemmaref[1]{\ifcsdef{@itemlabel@lemma-#1}{%
    \hyperref[#1]{\autoref*{\csuse{@itemlabel@lemma-#1}}\,(\ref*{#1})}%
  }{\autoref{#1}}}
\newcommand\lemmarefshort[1]{\ifcsdef{@itemlabel@lemma-#1}{%
    \hyperref[#1]{Lem.\,\ref*{\csuse{@itemlabel@lemma-#1}}\,(\ref*{#1})}%
  }{Lem.\,\ref{#1}}}

\mdfdefinestyle{proofstyle}{%
  backgroundcolor=black!4!white,
  innertopmargin=3pt,
  innerbottommargin=3pt,
  innerleftmargin=3pt,
  innerrightmargin=3pt,
  linewidth=0pt
}

\mdfdefinestyle{claimproofstyle}{%
  backgroundcolor=black!8!white,
  innertopmargin=0pt,
  innerbottommargin=3pt,
  innerleftmargin=3pt,
  innerrightmargin=3pt,
  leftmargin=10pt,
  rightmargin=10pt,
  % linewidth=0pt
}

\newenvironment{proof}[1][]{%
  \begin{mdframed}[style=proofstyle]%
    \begin{trivlist}%
    \item \textit{Proof\ifx\proof#1\proof\else\ #1\fi. }%
    }{
      \qed\global\let\qed\qedmacro
    \end{trivlist}
  \end{mdframed}}%

\newenvironment{claimproof}{%
  \let\qedbox\qedboxclaim
  \begin{mdframed}[style=claimproofstyle]%
    \begin{trivlist}%
    \item \textit{Proof of claim. }%
    }{
      \qed\global\let\qed\qedmacro
    \end{trivlist}
  \end{mdframed}}%

\newenvironment{claimproofstart}{%
  \let\qedbox\qedboxclaim
  \begin{mdframed}[style=claimproofstyle]%
    \begin{trivlist}%
    \item \textit{Proof of claim. }%
    }{
    \end{trivlist}
  \end{mdframed}}%

\newenvironment{claimproofend}{%
  \let\qedbox\qedboxclaim
  \begin{mdframed}[style=claimproofstyle]%
    \begin{trivlist}%
    \item%
    }{
      \qed\global\let\qed\qedmacro
    \end{trivlist}
  \end{mdframed}}%



% \showafter{year}{month}{day}{text} evaluates to {text} starting from year/month/day
\newcommand\showafter[4]{%
  \ifnum\year>#1\relax
    #4% today.year > args.year
  \else
    \ifnum\year=#1\relax
    % today.year = args.year
      \ifnum\month>#2\relax
      % today.month > args.month
        #4%
      \else
        \ifnum\month=#2\relax
        % today.month = args.month
          \ifnum\day>#3\relax
          % today.day >= args.day
            #4%
          \else
            \ch@removeduplicatespace
          \fi
        \else
          \ch@removeduplicatespace
        \fi
      \fi
    \else
      \ch@removeduplicatespace
    \fi
  \fi}


\let\textttOLD\texttt
\def\texttt#1{\textttOLD{\frenchspacing #1}}

\makeatletter
\newcommand\qedboxclaim{\ensuremath\diamond}
\newcommand\qedbox{\m@th$\Box$}
\newcommand\qedmacro{\hfill\qedbox}
\global\let\qed\qedmacro
\newcommand\skipqed{\global\let\qed\empty}
\newcommand\mathQED{\tag*{\qedbox}\skipqed}
\newcommand\txtrel[1]{\stackrel{\hskip-1in\text{\tiny#1}\hskip-1in}}
\newcommand\eqrefrel[1]{\txtrel{\eqref{#1}}}
\newcommand\starrel{\txtrel{$(*)$}}
\newcommand\tristarrel{\txtrel{$\scriptscriptstyle (\!*\!*\!*\!)$}}
\newcommand\fourstarrel{\txtrel{$\scriptscriptstyle (\!*\!*\!*\!*\!)$}}
\newcommand\starstarrel{\txtrel{$(**)$}}
\newcommand\boardpic[1]{\par{\centering\includegraphics[keepaspectratio=true,width=\hsize,height=2.5in]{#1}\par}}
\newcommand\rimplies{\DOTSB\;\Longleftarrow\;}
\newcommand\sublemmaref[2]{\autoref{#1}\,\eqref{sub#1:#2}}
\DeclareRobustCommand\autorefshort[1]{%
  \def\lemmaautorefname{Lem.\!}%
  \autoref{#1},
  p.\,\pageref{#1}}
\newcommand\bit{\{0,1\}}
\newcommand\bits[1]{\bit^{#1}}

\def\parenthesis@resizecommand@open{}
\def\parenthesis@resizecommand@close{}
\def\parenthesis@#1#2#3#4#5{%
  \global\let\parenthesis@resizecommand@open\empty
  \global\let\parenthesis@resizecommand@close\empty
  #1#3%
  {#5}%
  #2#4%
}
\DeclareRobustCommand\parenthesis[3]{%
  \expandafter\expandafter\expandafter
  \parenthesis@\expandafter\expandafter\expandafter{\expandafter\parenthesis@resizecommand@open\expandafter}\expandafter{\parenthesis@resizecommand@close}{#1}{#2}{#3}}


% #1=bigl #2=bigr #3=( #4=txt #5=) #6=txt #7=( #8=txt #9=)
\def\double@parenthesis@#1#2#3#4#5#6#7#8#9{%
  \global\let\parenthesis@resizecommand@open\empty
  \global\let\parenthesis@resizecommand@close\empty
  #1#3{#4}#2#5%
  {#6}%
  #1#7{#8}#2#9%
}

\DeclareRobustCommand\doubleParenthesis[7]{%
  \expandafter\expandafter\expandafter
  \double@parenthesis@\expandafter\expandafter\expandafter{\expandafter\parenthesis@resizecommand@open\expandafter}\expandafter{\parenthesis@resizecommand@close}{#1}{#2}{#3}{#4}{#5}{#6}{#7}}


\DeclareRobustCommand\resize@next@paren[2]{%
  \gdef\parenthesis@resizecommand@open{#1}%
  \gdef\parenthesis@resizecommand@close{#2}%
}

\newcommand\paren{\parenthesis()}
\newcommand\braces{\parenthesis\{\}}
\newcommand\brackets{\parenthesis[]}

\newcommand\pb{\resize@next@paren\bigl\bigr}
\newcommand\pbb{\resize@next@paren\biggl\biggr}
\newcommand\plr{\resize@next@paren\left\right}
\newcommand\pB{\resize@next@paren\Bigl\Bigr}

\newlistof{rule}{rule}{{List of rules}}
\renewcommand\cftruletitlefont{\section*}
\newcommand\rulestrut{}
\newcommand\rulespace{}
\newcommand\RULE[4][]{%
  \inferrule[\rulestrut{#2\ifx\norulelemmalink\undefined
    \textsuperscript{\normalfont\tiny[\autorefshort{rule-lemma:#2}]}\fi}%
    \refstepcounter{rule}%
    \label{rule:#2}%
    \index{#2@\textsc{#2} (rule)}%
    \addcontentsline{rule}{rule}{\textsc{#2}%
      \ifx\@nil#1\@nil\else\space -- #1\fi}
  ]{#3}{#4}\rulespace%  
}
\newcommand\ERULE[4][]{%
  \begin{mdframed}[style=theoremstyle]%
    \RULE[{#1}]{#2}{#3}{#4}
  \end{mdframed}
}
\newcommand\RULEX[4][]{%
  \inferrule[\rulestrut{#2}%
      \ifx\@nil#1\@nil\else\space -- #1\fi]{#3}{#4}\rulespace%  
}
\newcommand\RULEY[2]{%
  \inferrule{\rulestrut #1}{#2}\rulespace%  
}
\newenvironment{ruleblock}{%
  \begin{center}%
    \def\rulestrut{\vrule height 1.3\baselineskip width 0pt\relax}%
    \def\rulespace{\qquad}%
    \noindent
  }{%
  \end{center}}
  
\newcommand\refrule[1]{\hyperref[rule:#1]{\hbox{\textsc{#1}}} rule}
\newcommand\ruleref[1]{\hyperref[rule:#1]{rule \hbox{\textsc{#1}}}}
\newcommand\rulerefx[1]{\hyperref[rule:#1]{\hbox{\textsc{#1}}}}
\newcommand\Ruleref[1]{\hyperref[rule:#1]{Rule \hbox{\textsc{#1}}}}


%\newcommand\butter[2]{\basis{#1}\bra{#2}}
%\newcommand\selfbutter[2]{\proj{\basis{#1}{#2}}}

%\declare{macro=\varcard, code=\kappa, 
%  description={Upper bound for cardinality of variable types}}

\declare{macro=\abs, argspec=[1], code=\parenthesis\lvert\rvert{#1},
  placeholder=\abs x, nopage=true,
  description=Absolute value of $x$ / cardinality of set $x$}
%\declare{macro=\babs, argspec=[1], code={\bigl\lvert#1\bigr\rvert}, 
%  variantof=\abs}

\declare{macro=\qu, argspec=[1], code=#1^\mathsf{qu},
  placeholder=\qu V,
  description={Quantum variables in $V$}}
\declare{macro=\cl, argspec=[1], code=#1^\mathsf{cl},
  placeholder=\cl V,
  description={Classical variables in $V$}}

\declare{macro=\fv, argspec=[1], code=\mathit{fv}\paren{#1},
  placeholder=\fv e,
  description={Free variables in an expression $e$ (or program)}}

\declare{macro=\typev, argspec=[1], code=\mathsf{Type}_{#1},
  placeholder=\typev v,
  description={Type of variable $v$}}
\declare{macro=\types, argspec=[1], code=\mathsf{Type}^\mathsf{set}_{#1},
  placeholder=\types X,
  description={Type of a set $V$ of variables}}
\declare{macro=\typel, argspec=[1], code=\mathsf{Type}^\mathsf{list}_{#1},
  placeholder=\typel V,
  description={Type of a list $V$ of variables}}
\declare{macro=\typee, argspec=[1], code=\mathsf{Type}^\mathsf{exp}_{#1},
  placeholder=\typee e,
  description={Type of an expression $e$}}

\declare{macro=\denotee, argspec=[2], code=\parenthesis\llbracket\rrbracket{#1}_{#2},
  placeholder=\denotee em,
  description={Denotation of a classical expression $e$, evaluated on classical memory $m$}}

%\declare{macro=\denoteex, argspec=[1], code=\llbracket#1\rrbracket,
%  variantof=\denotee}

\declare{macro=\bc, code=\mathbf c, nopage=true,
  variable=true,
  placeholder={\bc,\bd},
  description={A program}}
% \declare{macro=\bd, code=\mathbf d, nopage=true,
%   variable=true,
%   description={A program}}
\newcommand\bd{\mathbf d}
\newcommand\be{\mathbf e}

\declare{macro=\denotc, argspec=[1], code={\parenthesis\llbracket\rrbracket{#1}},
  placeholder={\denotc \bc},
  description={Denotation of a program $\bc$}}
% \declare{macro=\denotcl, argspec=[1], code={\parenthesis\llbracket\rrbracket{#1}_\mathbf{class}},
%   placeholder={\denotcl \bc},
%   description={Classical denotation of a program $\bc$}}

\declare{macro=\Skip, code=\mathbf{skip},
  description={Program that does nothing}}

\declare{macro=\langif, argspec=[3], code={\mathbf{if}\ #1\ \mathbf{then}\ #2\ \mathbf{else}\ #3},
  placeholder=\langif e{c_1}{c_2},
  description=Statement: If (conditional)}
%\declare{macro=\langifx, argspec=[2], code={\mathbf{if}\ #1\ \mathbf{then}\ #2},
%  variantof=\langif}
%\declare{macro=\langifkw, code={\mathbf{if}},
%  variantof=\langif}

\declare{macro=\while, argspec=[2], code={\mathbf{while}\ #1\ \mathbf{do}\ #2},
  placeholder=\while ec,
  description=Statement: While loop}
%\declare{macro=\whilekw, code={\mathbf{while}},
%  variantof=\while}
\newcommand\whilep[2]{\while{#1}{\{#2\}}}

\declare{macro=\sample, argspec=[2],
  code={#1\stackrel{{\scriptstyle{}\smash\$}}\leftarrow #2},
  placeholder=\sample \xx e,
  description={Statement: Sample $\xx$ according to distribution $e$}}

\declare{macro=\Qinit, argspec=[2],
  code={#1\stackrel{{\scriptstyle{\smash{\mathfrak q}}}}\leftarrow #2},
  placeholder=\Qinit{\qq_1\dots \qq_n}{e},
  description={Statement: Initialize $\qq_1,\dots,\qq_n$ with quantum state $e$}}
\declare{macro=\Qapply, argspec=[2], code={\mathbf{apply}\ #1\ \mathbf{to}\ #2},
  placeholder=\Qapply{\qq_1\dots \qq_n}{U},
  description={Statement: Apply unitary/isometry $U$ to quantum registers $\qq_1\dots \qq_n$}}

\declare{macro=\Qmeasure, argspec=[3], code={#1 \leftarrow \mathbf{measure}\ #2\ \mathbf{with}\ #3},
  placeholder=\Qmeasure{\xx}{\qq_1\dots\qq_n}{e},
  description={Statement: Measure quantum variables $\qq_1\dots\qq_n$ with measurement $e$}}

% \declare{macro=\bool, code=\mathbb B,
%   description={Booleans. $\bool=\{\true,\false\}$}}

\declare{macro=\elltwo, argspec=[1], code={\ell^2(#1)},
  placeholder=\elltwo B,
  description={Hilbert space with basis indexed by $B$}}
\declare{macro=\elltwov, argspec=[1], code={\ell^2\parenthesis[]{#1}},
  placeholder=\elltwov V,
  description={$\elltwo{\types V}$ -- Hilbert space with basis $\types V$}}

% \declare{macro=\ellone, argspec=[1], code={\mathbf D(#1)},
%   placeholder=\ellone B,
%   description={Distributions on $B$}}
% \declare{macro=\ellonev, argspec=[1], code={\mathbf D[#1]},
%   placeholder=\ellonev V,
%   description={$\ellone{\types V}$ -- Distributions on $\types V$}}

% \declare{macro=\iso, argspec=[1], code=\mathbf{Iso}(#1),
%   placeholder={\iso{X,Y}, \iso X},
%   description={Isometries from $\elltwo X$ to $\elltwo Y$ (on $\elltwo X$)}}
% \declare{macro=\isov, argspec=[1], code={\mathbf{Iso}[#1]},
%   placeholder={\isov{V,W}, \iso V},
%   description={Isometries from $\elltwov V$ to $\elltwov W$ (on $\elltwov V$)}}

% \declare{macro=\uni, argspec=[1], code=\mathbf{U}(#1),
%   placeholder={\uni{X,Y}, \uni X},
%   description={Unitaries from $\elltwo X$ to $\elltwo Y$ (on $\elltwo X$)}}
% \declare{macro=\univ, argspec=[1], code={\mathbf{U}[#1]},
%   placeholder={\univ{V,W}, \uni V},
%   description={Unitaries from $\elltwov V$ to $\elltwov W$ (on $\elltwov V$)}}

% \declare{macro=\distr, argspec=[1], code=\mathbf D^{\leq1}(#1),
%   placeholder=\distr X,
%   description={Sub-probability distributions over $X$}}
% \declare{macro=\distrv, argspec=[1], code=\mathbf D^{\leq1}[#1],
%   placeholder=\distrv V,
%   description={Sub-probability distributions over variables $V$}}

% \declare{macro=\setC, code=\mathbb C,
%   description={Complex numbers}}
% \declare{macro=\setR, code=\mathbb R,
%   description={Real numbers}}
% \declare{macro=\setRpos, code=\mathbb R_{\geq0},
%   description={Non-negative real numbers}}

% \declare{macro=\tracecl, argspec=[1], code=\mathbf T(#1),
%   placeholder={\tracecl X},
%   description=Trace class operators on $\elltwo X$}
% \declare{macro=\tracepos, argspec=[1], code=\mathbf T^+(#1),
%   placeholder={\tracepos X},
%   description=Positive trace class operators on $\elltwo X$}
\declare{macro=\tensor, code=\otimes,
  placeholder={A\otimes B},
  description={Tensor product of vectors/operators $A$ and $B$}}

% \declare{macro=\traceclv, argspec=[1], code=\mathbf T[#1],
%   placeholder={\traceclv V},
%   description=Trace class operators on $\elltwov V$}
% \declare{macro=\traceposv, argspec=[1], code=\mathbf T^+[#1],
%   placeholder={\traceposv V},
%   description=Positive trace class operators on $\elltwov V$}
% \declare{macro=\traceclcq, argspec=[1], code=\mathbf T_{\mathit{cq}}[#1],
%   placeholder={\traceclcq V},
%   description=Trace class cq-operators on $\elltwov V$}

% \declare{macro=\pointdistr, argspec=[1],
%   code={\delta_{#1}},
%   placeholder=\pointdistr{x},
%   description={Point distribution: returns $x$ with probability $1$}}

\declare{macro=\restricte, argspec=[1], code=\mathord\downarrow_{#1},
  placeholder=\restricte e(\rho),
  description={Restrict state/distribution $\rho$ to the case $e=\true$ holds}}
%\newcommand\restrictno[2]{#1}

\declare{macro=\seq, argspec=[2], code=#1;#2,
  placeholder=\bc;\bd,
  description={Sequential composition of programs}}


% \declare{macro=\pointstate, argspec=[2],
%   code={\delta_{#1}(#2)},
%   placeholder=\delta_V(x),
%   description={Point distribution as density operator}}
\newcommand\pointstate[2]{\proj{\basis{#1}{#2}}}

\declare{macro=\true, code=\mathtt{true}, nopage=true,
  description={Truth value ``true''}}
\declare{macro=\false, code=\mathtt{false}, nopage=true,
  description={Truth value ``false''}}

% \declare{macro=\traceposcq, argspec=[1], code=\mathbf T^+_{\mathit{cq}}[#1],
%   placeholder={\traceposcq V},
%   description=Positive trace class cq-operators on $\elltwov V$}

% \declare{macro=\qlift, argspec=[1], code=\mathsf{lift}\paren{#1},
%   placeholder=\qlift\mu,
%   description=Transforms a distribution $\mu$ into a density operator}

\declare{macro=\lift, argspec=[2], code={#1\textrm\guillemotright#2},
  placeholder=\lift AQ,
  description={Lifts operator or subspace to variables $Q$}}

%\declare{macro=\compl, argspec=[1], code=#1^{\complement},
%  placeholder=\compl X,
%  description=Complement of the set $X$}

\declare{macro=\calE, code=\mathcal E, variable=true,
  description=A superoperator}
\newcommand\calF{\mathcal F}
\newcommand\calM{\mathcal M}
\newcommand\calL{\mathcal L}

% \declare{macro=\bounded, argspec=[1], code=\mathbf B(#1),
%   placeholder={\bounded{X,Y}},
%   description=Bounded linear operators from $\elltwo X$ to $\elltwo Y$}
% \declare{macro=\boundedleq, argspec=[1], code=\mathbf B^{\leq1}(#1),
%   placeholder={\boundedleq{X,Y}},
%   description=Bounded linear operators with operator norm $\leq1$}
% \declare{macro=\boundedv, argspec=[1], code=\mathbf B[#1],
%   placeholder=\boundedv{V,W},
%   description={Bounded linear operators from $\elltwov V$ to $\elltwo W$}}

\declare{macro=\idv, argspec=[1], code=\mathit{id}_{#1},
  placeholder=\idv \VV,
  description=Identity over variables $\VV$}
\declare{macro=\id, code=\mathit{id},
  description=Identity}

\declare{macro=\adj, argspec=[1], code=#1^*,
  placeholder={\adj A},
  description={Adjoint of the operator $A$}}

%\newcommand\basisOLD[1]{\lvert #1\rangle}
\declare{macro=\basis, argspec=[2], code={\parenthesis\lvert\rangle{#2}_{\!\scriptscriptstyle{#1}}},
  placeholder={\basis{} b, \basis V b},
  description={Basis vector in Hilbert space $\elltwov V$}}
%\declare{macro=\bra, argspec=[1], code={\langle #1\lvert},
%  placeholder=\bra b,
%  description={$\adj{\basis b}$, adjoint of basis vector $\basis b$}}

% \declare{macro=\hoarev, argspec=[4], code={\{#1\}#2\{#3\}^{#4}},
%   placeholder=\hoarev F\bc GV,
%   description={Possibilistic Hoare judgement (variables $V$ omitted if clear)}}
% \declare{macro=\hoare, argspec=[3], code={\{#1\}#2\{#3\}},
%   variantof=\hoarev}

\declare{macro=\rhl, argspec=[4],
  % code={\{#1\}#2\pmb\sim#3\{#4\}},
  code={\doubleParenthesis\{{#1}\}{#2\pmb\sim#3}\{{#4}\}},
  placeholder=\rhl F\bc{\bc'} G,
  description={Quantum relational Hoare judgment}}
% \declare{macro=\rhlfirst, argspec=[4],
%   % code={\{#1\}#2\pmb\sim#3\{#4\}},
%   code={\doubleParenthesis\{{#1}\}{#2\pmb\sim#3}\{{#4}\}_\mathsf{nonsep}},
%   placeholder=\rhlfirst F\bc{\bc'} G,
%   description={qRHL judgment, non-separable definition}}
% \declare{macro=\rhlunif, argspec=[4],
%   % code={\{#1\}#2\pmb\sim#3\{#4\}},
%   code={\doubleParenthesis\{{#1}\}{#2\pmb\sim#3}\{{#4}\}_\mathsf{uniform}},
%   placeholder=\rhlunif F\bc{\bc'} G,
%   description={qRHL judgment, uniform definition}}
% %\declare{macro=\rhlv, argspec=[6], code={\{#1\}#2\sim#3\{#4\}^{#5,#6}},
% %  variantof=\rhlv}
% \declare{macro=\prhl, argspec=[4],
%   % code={\{#1\}#2\pmb\sim#3\{#4\}},
%   code={\doubleParenthesis\{{#1}\}{#2\pmb\sim#3}\{{#4}\}_\mathsf{class}},
%   placeholder=\prhl F\bc{\bc'} G,
%   description={pRHL judgement (classical)}}

\declare{macro=\partr, argspec=[2], 
  code=\mathord{\operatorname{tr}\ifx\@nil#1\@nil\else^{\scriptscriptstyle[#1]}\fi_{\scriptscriptstyle #2}},
  placeholder=\partr VW(\rho),
  description={Partial trace, keeping variables $V$, dropping variables $W$}}

\declare{macro=\im, code=\operatorname{im},
  placeholder=\im A,
  description={Image of $A$}}
\declare{macro=\dom, code=\operatorname{dom},
  placeholder=\dom f,
  description={Domain of $f$}}

\declare{macro=\norm, argspec=[1], code={\parenthesis\lVert\rVert{#1}},
  placeholder=\norm x, description={$\ell_2$-norm of vector $x$, or operator-norm}}

% % From: https://tex.stackexchange.com/a/193126

% % Math symbol font matha
% \DeclareFontFamily{U}{matha}{\hyphenchar\font45}
% \DeclareFontShape{U}{matha}{m}{n}{
%       <5> <6> <7> <8> <9> <10> gen * matha
%       <10.95> matha10 <12> <14.4> <17.28> <20.74> <24.88> matha12
%       }{}
% \DeclareSymbolFont{matha}{U}{matha}{m}{n}
% \DeclareFontSubstitution{U}{matha}{m}{n}

% % Math symbol font mathb
% \DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
% \DeclareFontShape{U}{mathx}{m}{n}{
%       <5> <6> <7> <8> <9> <10>
%       <10.95> <12> <14.4> <17.28> <20.74> <24.88>
%       mathx10
%       }{}
% \DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
% \DeclareFontSubstitution{U}{mathx}{m}{n}

% % Symbol definition
% \DeclareMathDelimiter{\vvvert}{0}{matha}{"7E}{mathx}{"17}


% \newcommand\onorm[1]{\parenthesis\vvvert\vvvert{#1}}


\declare{macro=\tr, code=\operatorname{tr},
  placeholder=\tr M,
  description={Trace of matrix/operator $M$}}

\declare{macro=\CL, argspec=[1], code=\mathfrak{Cla}\parenthesis[]{#1},
  placeholder=\CL e,
  description={Classical predicate meaning $e=\true$}}

\declare{macro=\SPAN, code={\operatorname{span}},
  placeholder=\SPAN A,
  description={Span, smallest subspace containing $A$}}
% \newcommand\SPANO[1]{\SPAN\{#1\}}

\declare{macro=\quanteq, code={\equiv_\mathsf{quant}},
  placeholder=X_1\quanteq X_2,
  description={Equality of quantum variables $X_1$ and $X_2$}}

\declare{macro=\proj, argspec=[1], code={\mathbf{proj}\paren{#1}},
  placeholder=\proj x,
  description={Projector onto $x$. More precisely, $x\adj x$}}

\declare{macro=\toE, argspec=[1], code={\mathbf{toE}\paren{#1}},
  placeholder=\toE U,
  description={Superoperator corresponding to $U$. I.e. $\toE U(\rho):=U\rho\adj U$.}}

\declare{macro=\prafter, argspec=[3], code={\Pr\parenthesis[]{#1 : #2(#3)}},
  placeholder=\prafter e\bc\rho,
  description={Probability that $e$ holds after running $\bc$ on initial state $\rho$}}

% \declare{macro=\Urename, argspec=[1], code={U_{\mathit{rename},#1}},
%   placeholder=\Urename{\sigma},
%   description={Unitary: Renames variables according to bijection $\sigma$}}


% \declare{macro=\Erename, argspec=[1], code={\calE_{\mathit{rename},#1}},
%   placeholder=\Erename{\sigma},
%   description={cq-superoperator: Renames variables according to bijection $\sigma$}}

\declare{macro=\subst, argspec=[2], code=#1#2,
  placeholder={\subst e\sigma, \subst\bc\sigma},
  description={Apply variable substitution $\sigma$ to expression $e$}}

\declare{macro=\substi, argspec=[2], code=#1\{#2\},
  placeholder=\substi e{f/\xx},
  description={Substitute $f$ for variable $\xx$ in $e$}}

% \declare{macro=\restrict, argspec=[2], code=#1|_{#2},
%   placeholder=\restrict fM,
%   description={Restriction of function $f$ to domain $M$}}

\declare{macro=\vv, code=\mathbf v,
  placeholder={\vv,\ww},
  description={A program variable (classical or quantum)}}
\newcommand\ww{\mathbf w}

\declare{macro=\xx, code=\mathbf x,
  placeholder={\xx,\yy},
  description={A classical program variable}}
\newcommand\yy{\mathbf y}
%\declare{macro=\yy, code=\mathbf y,
%  description={A classical program variable}}
%\declare{macro=\zz, code=\mathbf z,
%  description={A classical program variable}}
\declare{macro=\qq, code=\mathbf q,
  placeholder={\qq,\rr},
  description={A quantum program variable}}
\newcommand\rr{\mathbf r}
% \declare{macro=\rr, code=\mathbf r,
%   description={A quantum program variable}}


\declare{macro=\upd, argspec=[3], code={#1(#2:=#3)},
  placeholder=\upd fxy,
  description={Function update, i.e., $(\upd fxy)(x)=y$}}

\newcommand\localkw{\mathbf{local}}
\declare{macro=\local, argspec=[2],
  % code={\mathbf{local}\ #1\ \mathbf{in}\ #2},
  % code={\braces{\mathbf{local}\ #1;\ #2}},
  code={{\localkw\ #1; #2}},
  placeholder=\local V\bc,
  description={Program: $\bc$ with local variables $V$}}
\newcommand\locala[1]{\mathbf{local}\ #1}
\newcommand\localp[2]{\paren{\local{#1}{#2}}}
\newcommand\localpp[2]{{\local{#1}{\paren{#2}}}}

\declare{macro=\LOCAL, argspec=[2],
  code={\mathbf{Local}_{#1}\brackets{#2}},
  placeholder={\LOCAL\vv\calE},
  description={Superoperator $\calE$ with variable $\vv$ made local}}

\declare{macro=\assign, argspec=[2], code={#1\leftarrow #2},
  placeholder=\assign xe,
  description={Program: assigns expression $e$ to $x$}}

\declare{macro=\suppd, code=\operatorname{supp},
  placeholder=\suppd \mu,
  description={Support of distribution $\mu$}}
\declare{macro=\suppo, code=\operatorname{\mathbf{supp}},
  placeholder=\suppo M,
  description={Support of an operator $M$}}

\declare{macro=\marginal, argspec=[2], code={\mathsf{marginal}_{#1}\parenthesis(){#2}},
  placeholder=\marginal i\mu,
  description={$i$-th marginal distribution of $\mu$}}

\declare{macro=\orth, argspec=[1], code={#1^\bot},
  placeholder=\orth S,
  description={Orthogonal complement of subspace $S$}}

% \declare{macro=\calH, code=\mathcal H,
%   description={A Hilbert space}}

% \declare{macro=\pinv, argspec=[1], code=#1^+,
%   placeholder=\pinv A,
%   description={Moore-Penrose pseudoinverse}}

% \declare{macro=\idx, argspec=[1], code=\operatorname{idx}_{#1},
%   placeholder={\idx 1\bc, \idx 1 e},
%   description={Add index $1$ to every variables in $\bc$ or $e$}}

% \declare{macro=\Meas, argspec=[2], code={\mathbf{Meas}(#1,#2)},
%   placeholder=\Meas DE,
%   description={Projective measurements on $\elltwo E$ with outcomes in $D$}}

% \declare{macro=\Uvarnames, argspec=[1], code=U_{\mathit{vars},#1},
%   placeholder=\Uvarnames{Q},
%   description={Canonical isomorphism between $\elltwo{\typel Q}$
%     and $\elltwov{\types Q}$ for a list $Q$}}

% \declare{macro=\leftim, argspec=[1], code=\overleftarrow\im\, #1,
%   placeholder=\leftim R,
%   description={Left image of relation $R$}}

% \declare{macro=\rightim, argspec=[1], code=\overrightarrow\im\, #1,
%   placeholder=\rightim R,
%   description={Right image of relation $R$}}

\declare{macro=\spaceat, argspec=[2], code=#1\div#2,
  placeholder=\spaceat A\psi,
  description={Part of $A$ containing $\psi$}}

% \declare{macro=\memuni, argspec=[1], code=#1,
%   placeholder=\memuni{m_1m_2},
%   description={Union (concatenation) of memories $m_1$, $m_2$}}

% \declare{macro=\powerset, argspec=[1], code=2^{#1},
%   placeholder=\powerset M,
%   description={Powerset of $M$}}

% \declare{macro=\floor, argspec=[1], code=\parenthesis\lfloor\rfloor{#1},
%   placeholder=\floor x,
%   description={$x$ rounded down to the next integer}}

%\declare{macro=\sampleset, code=\in_{\scriptstyle{}\$},
%  placeholder=x\sampleset M,
%  description={$x$ uniformly sampled from $M$}}
% \declare{macro=\AdvROR, code=\mathrm{Adv}_\mathrm{ROR},
%   placeholder=\AdvROR^{A_1A_2}(\eta),
%   description={Advantage of adversary $A_1,A_2$ in ROR-OT-CPA game with security parameter $\eta$}}
% \declare{macro=\AdvPRG, code=\mathrm{Adv}_\mathrm{PRG},
%   placeholder=\AdvPRG^{A}(\eta),
%   description={Advantage of adversary $A$ in PRG-OT-CPA game with security parameter $\eta$}}
% \declare{macro=\Time, code=\mathrm{Time},
%   placeholder=\Time(A),
%   description={Worst-case runtime of $A$}}


% \declare{macro=\circexp, code=\circ_e,
%   placeholder=a \circexp b,
%   description={Composition of expressions $a,b$ as relations}}
% \declare{macro=\circrel, code=\circ,
%   placeholder=R_1 \circrel R_2,
%   description={Composition of relations}}

% \declare{macro=\setN, code=\mathbb N,
%   description={Natural numbers}}

\declare{macro=\XX, code=\mathbf X,
  placeholder={\XX,\YY},
  description={List/set of classical program variables}}
\newcommand\YY{\mathbf Y}
%\newcommand\ZZ{\mathbf Z}

\declare{macro=\QQ, code=\mathbf Q,
  placeholder={\QQ, \RR, \SSS},
  description={List/set of quantum program variables}}
\newcommand\RR{\mathbf R}
\newcommand\SSS{\mathbf S}

\declare{macro=\VV, code=\mathbf V,
  placeholder={\VV,\WW},
  description={List/set of program variables}}
\newcommand\WW{\mathbf W}

\declare{macro=\initial, argspec=[1], code={\bullet_{#1}},
  placeholder=\initial\vv,
  description={Default value for variable $\vv$}}
\declare{macro=\rhoinit, argspec=[1], code={\rho^\bullet_{#1}},
  placeholder=\rhoinit\vv,
  description={Density operator with default value for variable $\vv$}}
%\declare{macro=\psiinit, argspec=[1], code={\psi^\bullet_{#1}},
%  placeholder=\psiinit\vv,
%  description={Quantum state with default value for variable $\vv$}}
\newcommand\psiinit[1]{\basis{#1}{\initial{}}}

\declare{macro=\swap, argspec=[2], code={\mathsf{SWAP}_{#1\leftrightarrow#2}},
  placeholder=\swap\vv{\vv'},
  description={Unitary swapping $\vv$, $\vv'$}}

\newcommand\swapcop[1]{\swap{#1}{#1'}}

% \declare{macro=\swapcop, argspec=[1], code={\mathsf{SWAP}^\mathbf{copy}_{#1}},
%   placeholder=\swapcop\vv,
%   description={Unitary swapping $\vv$ and $\cop\vv$}}

% \declare{macro=\cop, argspec=[1], code=#1^\mathbf{copy},
%   placeholder=\cop\vv,
%   description={Copy of variable $\vv$}}

% \declare{macro=\sandwich, argspec=[2], code={#1\star #2},
%   placeholder=\sandwich U\rho,
%   description={Short for $U\rho \adj U$}}

% \declare{macro=\equpto, argspec=[1], code=\cong_{#1},
%   placeholder=\equpto\VV,
%   description={Semantically equivalent up to variables $\VV$}}

\declare{macro=\init, argspec=[1], code=\mathbf{init}\ #1,
  placeholder=\init\vv,
  description={Program: Initialize $\vv$ with default value}}
\newcommand\initkw{\mathbf{init}}

\declare{macro=\PA, code=\mathsf A,
  placeholder={\PA,\PB,\PC},
  description={(Quantum) predicates}}
\newcommand\PB{\mathsf B}
\newcommand\PR{\mathsf R}
\newcommand\PC{\mathsf C}

\declare{macro=\hole, argspec=[1], code=\Box_{#1},
  placeholder=\hole i,
  description={$i$-th hole in a context}}

% \declare{macro=\holelocal, argspec=[1], code=\mathsf{locals}^\Box\paren{#1},
%   placeholder=\holelocal C,
%   description={Variables that are local over the holes of $C$}}

% \declare{macro=\psubst, argspec=[3], code=#1\braces{#2/#3},
%   placeholder=\psubst\PA\VV\WW,
%   description={Predicate $\PA$ with $\WW$ substituted by $\VV$}}

\declare{macro=\VVall, code=\VV^{\mathbf{all}},
  description={Set of all program variables that can be used in the execution of a program}}

\declare{macro=\written, argspec=[1], code=\mathit{written}\paren{#1},
  placeholder=\written\bc,
  description=Variables written by $\bc$}

\declare{macro=\inner, argspec=[1], code=\mathit{inner}\paren{#1},
  placeholder=\inner C,
  description=Inner variables of context $C$}

\declare{macro=\covered, argspec=[1], code=\mathit{covered}\paren{#1},
  placeholder=\covered C,
  description=Covered variables of context $C$}

\declare{macro=\overwr, argspec=[1], code=\mathit{overwr}\paren{#1},
  placeholder=\overwr\bc,
  description=Overwritten variables of $\bc$}

% \declare{macro=\opon, argspec=[2], code={#1\,\mathbf{on}\,#2},
%   placeholder=\opon U\VV,
%   description={Operator $U$ applied to variables $\VV$}}

\declare{macro=\eqstate, code={=_\mathfrak q},
  placeholder={\VV\eqstate\psi},
  description={Predicate: $\VV$ is in state $\psi$}}

% \declare{macro=\quantin, code=\in_{\mathfrak q},
%   placeholder=\VV\quantin S,
%   description={Predicate: $\VV$ has a value in $S$}}

\declare{macro=\deneq, code={\stackrel{\textsf{d}}=},
  placeholder=\bc\deneq\bd,
  description={Denotational equivalence}}

\declare{macro=\Einit, argspec=[1], code={\calE^\textsf{init}_{#1}},
  placeholder=\Einit\vv,
  description={Superoperator initializing $\vv$}}

\declare{macro=\fullsubst, argspec=[2], code={#1\,^!#2},
  placeholder=\fullsubst\bc\sigma,
  description={Full substitution (incl.~local variables)}}

\declare{macro=\noconflict, argspec=[2], code={\mathit{no{}conflict}\paren{#1,#2}},
  placeholder=\noconflict\sigma\bc,
  description={Renaming $\bc$ with $\sigma$ leads to no free variable conflict}}

\newcommand\fsq{\tfrac1{\sqrt2}}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "localvars"
%%% TeX-PDF-mode: t 
%%% End: 

%  LocalWords:  Powerset

